Scalable adaptive algorithms for next-generation multiphase flow simulations

High-fidelity flow simulations are indispensable when analyzing systems exhibiting multiphase flow phenomena. The accuracy of multiphase flow simulations is strongly contingent upon the finest mesh resolution used to represent the fluid-fluid interfaces. However, the increased resolution comes at a higher computational cost. In this work, we propose algorithmic advances that aim to reduce the computational cost without compromising on the physics by selectively detecting key regions of interest (droplets/filaments) that require significantly higher resolution. The framework uses an adaptive octree-based meshing framework that is integrated with PETSc's linear algebra solvers. We demonstrate scaling of the framework up to 114,688 processes on TACC's Frontera. Finally, we deploy the framework to simulate one of the most resolved simulations of primary jet atomization. This simulation -- equivalent to 35 trillion grid points on a uniform grid -- is 64 times larger than the current state-of-the-art simulations and provides unprecedented insights into an important flow physics problem with a diverse array of engineering applications.

==> Sections/Methods/Challenges.tex <==
The parallel deployment of multiphase simulation comes up with its own set of challenges. As the simulation progress in time, the interface blooms, break into droplets, and forms complex regions and shapes. This leads to a significant increase in the mesh resolution as the time and simulation progress. We showcase one such simulation of primary jet atomization later in ~\secref{sec:Atomization}. With the increase in the mesh resolution, it is desirable to increase the number of processes accordingly.

We dump the files checkpoint files at frequent intervals. Once the checkpoint is reloaded, we can load it either from the same or larger number of processes. Specific care must be taken while loading with increased processor count. When the processor count is increased, \texttt{MPI\_Comm} is split into \texttt{active} and \texttt{inactive} communicators. The checkpoint is loaded with \texttt{active} communicators, and the mesh is created only within the \texttt{active} communicator. The \texttt{active} communicator has the size of the processes that dump the checkpoint files. Once a repartition or remeshing is triggered, the new mesh is then redistributed among all the available processes. The \texttt{inactive} communicators become \texttt{active} once the repartition or remeshing function is called.

==> Sections/RelatedWork.tex <==
In this work, we have shown the importance of identifying the key regions of interest and selectively refining those specific regions. The alternative approaches for accompanying the task can be through the route of determining the connected components ~\cite{harrison2015distributed}. However, the connected component is computationally more expensive and non--trivial to implement compared to the current approach. Additionally, connected component labeling is not enough to identify all the regions of interest, such as the thin filament, which is a part of the big structure (for example, \figref{fig:filament}). Furthermore, the proposed approach by ~\citet{harrison2015distributed} is limited to octree-based meshes, whereas the current approach in this work can be easily integrated into other numerical libraries with structured and unstructured meshes, as it solely relies on efficient ~\mvec{} computations -- a key component of scientific computations.

In the context of sharp interface capturing methods, there are advances in techniques, for example, in interface reconstruction~\citep{Lu2018, Chiodi2020}, moment-of-fluid~\citep{Jemison2015}, manifold death~\citep{Chirco2022} that also resolve try to resolve small structures. These techniques are, however, limited to sharp interface methods at the moment.  

==> Sections/Results/Refinement.tex <==
\subsection{Refinement \& Intergrid transfer}

Show the performance improvement for a simple bubble rise case.

==> Sections/Results/Tensor.tex <==
\subsection{Tensor}
Single processor improvements.
